PAM: Understanding Product Images in Cross Product Category Attribute Extraction

Understanding product attributes plays an important role in improving online shopping experience for customers and serves as an integral part for constructing a product knowledge graph. Most existing methods focus on attribute extraction from text description or utilize visual information from product images such as shape and color. Compared to the inputs considered in prior works, a product image in fact contains more information, represented by a rich mixture of words and visual clues with a layout carefully designed to impress customers. This work proposes a more inclusive framework that fully utilizes these different modalities for attribute extraction. Inspired by recent works in visual question answering, we use a transformer based sequence to sequence model to fuse representations of product text, Optical Character Recognition (OCR) tokens and visual objects detected in the product image. The framework is further extended with the capability to extract attribute value across multiple product categories with a single model, by training the decoder to predict both product category and attribute value and conditioning its output on product category. The model provides a unified attribute extraction solution desirable at an e-commerce platform that offers numerous product categories with a diverse body of product attributes. We evaluated the model on two product attributes, one with many possible values and one with a small set of possible values, over 14 product categories and found the model could achieve 15% gain on the Recall and 10% gain on the F1 score compared to existing methods using text-only features.

==> relatedwork.tex <==
\subsection{Value Extraction for Given Attributes}
Multiple works from e-commerce companies exist on extracting product
attributes from product textual description. For example, the open-tag
model \cite{zheng2018opentag} proposed to use a architecture of
Bi-direction LSTM model followed by conditional random field (CRF) to
tag attributes in product texts.  Since then, the industry has quickly
discovered that one model trained for one product type may not work
well for another product type due to data distribution difference. For
example, the size vocabulary for t-shirt is different from baby
diapers. On the other hand, it is too expensive to maintain a separate
model for each product type and each attribute
\cite{dong2020autoknow}. Hence one research focus is on training a
single model to accommodate multiple product types or attribute
values. In \cite{xu2019scaling}, the attribute name is converted into
an embedding with a BERT \cite{devlin2018bert} model which is used to
compute attention over product texts. In
\cite{karamanolakis2020txtract}, an auxiliary task of predicting
attribute type is used to improve the intermediate
representation. Product type is converted into Poincar\'e embedding to
compute attention in later layers. Instead of using LSTM model,
recently reference \cite{wang2020learning} concatenate the attribute
name and texts and feed it to a single BERT model.

Utilizing image to extract product attributes has received attention
recently in , for example, \cite{zhu2020multimodal} where a gated
attention layer to combine information from product image and text was
introduced. This work is different from \cite{zhu2020multimodal} in
that we consider texts in product images too which is shown to be
useful in product attributes.

\subsection{Visual Question Answering}

Our task is closely related to the visual question answering (VQA)
task hence our model is inspired by recent works in that field. Early
works in this field focus on the design of the design to merge
information from image and text modality, such as the bilinear
attention in \cite{kim2018bilinear}. The importance of the text in VQA
task was first recognized in \cite{singh2019towards} which proposed a
new benchmark dataset called textVQA. Reference \cite{hu2020iterative}
proposed to use transformers to support a more general form of
attention between image, image objects, image texts and
questions. This architecture is adopted and improved in later
works. Recently \cite{yang2020tap} introduced pretraining tasks to
this model architecture that boosted the state of art of textVQA
benchmark significantly.

The model we use is also adopted from \cite{hu2020iterative}. Our task
is different from text VQA \cite{hu2020iterative, yang2020tap} in that
there is an additional input of product description to the model and
the task also contains a challenge of designing a model that can adapt
to different product types. For example, the decoder in
\cite{hu2020iterative} chooses word from a vocabulary of high frequent
words in the answer set. In our task, this vocabulary is very
different for different product types, hence we made modification in
the decoder and the expected generated sequence to enable the model to
adapt to different product types.





